The different flavors of extragalactic jets: the role of relativistic flow deceleration

We perform three-dimensional numerical simulations of relativistic (with a Lorentz factor of 10), non magnetized jets propagating in a uniform density environment, in order to study the effect of the entrainment and the consequent deceleration. Our simulations investigate the jet propagation inside the galaxy core, where, most likely, the deceleration occurs more efficiently. We compare cases with different density and pressure ratios with respect to the ambient medium finding that low density jets are efficiently decelerated and reach a quasi steady state in which, over a length of 600 jet radii, slow down from highly to sub-relativistic velocities. At the opposite, denser jets keep highly relativistic velocity over the same length. We discuss these results in relation to the Faranoff Riley (FR) radio-sources classification. We infer that lower density jets can give rise to FR 0 and FR I radio-sources, while higher density jets may be connected to FR II radio-sources.

==> ref.tex <==
@ARTICLE{baldi19,
       author = {{Baldi}, Ranieri D. and {Capetti}, Alessandro and {Giovannini}, Gabriele},
        title = "{High-resolution VLA observations of FR0 radio galaxies: the properties and nature of compact radio sources}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: elliptical and lenticular, cD, galaxies: jets, galaxies: nuclei, radio continuum: galaxies, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2019,
        month = jan,
       volume = {482},
       number = {2},
        pages = {2294-2304},
          doi = {10.1093/mnras/sty2703},
archivePrefix = {arXiv},
       eprint = {1810.01894},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.482.2294B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{blandford78,
       author = {{Blandford}, R.~D. and {Rees}, M.~J.},
        title = "{Some comments on radiation mechanisms in Lacertids.}",
     keywords = {Astronomical Models, Bl Lacertae Objects, Dynamic Models, Luminous Intensity, Periodic Variations, Radiation Sources, Nonthermal Radiation, Plasma Radiation, Polarization Characteristics, Quasars, Radio Sources (Astronomy), Relativistic Effects, Synchrotron Radiation, Thermal Emission, Astrophysics, BL Lacertae Objects:Models, BL Lacertae Objects:Outbursts},
    booktitle = {BL Lac Objects},
         year = 1978,
       editor = {{Wolfe}, A.~M.},
        month = jan,
        pages = {328-341},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1978bllo.conf..328B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


